On a numerical upper bound for the extended Goldbach conjecture

The Goldbach conjecture states that every even number can be decomposed as the sum of two primes. Let $D(N)$ denote the number of such prime decompositions for an even $N$. It is known that $D(N)$ can be bounded above by $$ D(N) \leq C^* \Theta(N), \quad \Theta(N):= \frac{N}{\log^2 N}\prod_{\substack{p|N p>2}} \left( 1 + \frac{1}{p-2}\right)\prod_{p>2}\left(1-\frac{1}{(p-1)^2}\right) $$ where $C^*$ denotes Chen's constant. It is conjectured that $C^*=2$. In 2004, Wu showed that $C^* \leq 7.8209$. We attempted to replicate his work in computing Chen's constant, and in doing so we provide an improved approximation of the Buchstab function $\omega(u)$, \begin{align*} \omega(u)=1/u, & \quad (1\leq u\leq 2), (u \omega(u))'=\omega(u-1), & \quad (u\geq 2). \end{align*} based on work done by Cheer and Goldston. For each interval $[j,j+1]$, they expressed $\omega(u)$ as a Taylor expansion about $u=j+1$. We expanded about the point $u=j+0.5$, so $\omega(u)$ was never evaluated more than $0.5$ away from the center of the Taylor expansion, which gave much stronger error bounds. Issues arose while using this Taylor expansion to compute the required integrals for Chen's constant, so we proceeded with solving the above differential equation to obtain $\omega(u)$, and then integrating the result. Although the values that were obtained undershot Wu's results, we pressed on and refined Wu's work by discretising his integrals with finer granularity. The improvements to Chen's constant were negligible (as predicted by Wu). This provides experimental evidence, but not a proof, that were Wu's integrals computed on smaller intervals in exact form, the improvement to Chen's constant would be negligible. Thus, any substantial improvement on Chen's constant likely requires a radically different method to what Wu provided.

==> bibliography.tex <==

\begin{thebibliography}{88} % assuming between 10 and 99 references

 \bibitem{key1} Entry 1

 \bibitem{key2} Entry 2

 \bibitem{key3} Entry 3

 \bibitem{key4} Entry 4

 \bibitem{key5} Entry 5

 \bibitem{key6} Entry 6

 \bibitem{key7} Entry 7

 \bibitem{key8} Entry 8

 \bibitem{key9} Entry 9

 \bibitem{key10} Entry 10

\end{thebibliography}


==> biblo.tex <==
	@book{guy1994unsolved,
		title={Unsolved problems in number theory},
		author={Guy, R.K.},
		isbn={9780387942896},
		lccn={94215522},
		series={Problem books in mathematics},
		url={https://books.google.com.au/books?id=ZrwrAAAAYAAJ},
		year={1994},
		publisher={Springer-Verlag}
	}
	
		 @misc{ goldbachverify,
		 	author = {Tomás Oliveira e Silva},
		 	title = {{{Goldbach}} conjecture verification},
		 	url = {http://sweet.ua.pt/tos/goldbach.html},
		 	note = {[Online; accessed 31-January-2017]},
		 	year= {2017}
		 }
	 
	@article{ross1975chen,
	  title={On Chen's Theorem that Each Large Even Number has the Form $p_1+ p_2$ OR $p_1+ p_2 p_3$},
	  author={Ross, PM},
	  journal={Journal of the London Mathematical Society},
	  volume={2},
	  number={4},
	  pages={500--506},
	  year={1975},
	  publisher={Oxford University Press}
	}
	
	@article{helfgott2013ternary,
	  title={The ternary {{Goldbach}} conjecture is true},
	  author={Helfgott, Harald A},
	  journal={arXiv preprint arXiv:1312.7748},
	  year={2013}
	}
	
	@article{hardy1923some,
	  title={Some problems of ‘Partitio numerorum’; III: On the expression of a number as a sum of primes},
	  author={Hardy, Godfrey H and Littlewood, John E},
	  journal={Acta Mathematica},
	  volume={44},
	  number={1},
	  pages={1--70},
	  year={1923},
	  publisher={Springer}
	}
	
	@article{wu2004chen,
	  title={Chen's double sieve, {{Goldbach}}'s conjecture and the twin prime problem},
	  author={Wu, J},
	  journal={Acta Arithmetica},
	  volume={114},
	  pages={215--273},
	  year={2004}
	}
	
	@book{vinogradov1954method,
	  title={The method of trigonometrical sums in the theory of numbers},
	  author={Vinogradov, I.M.},
	  lccn={lc54003665},
	  url={https://books.google.com.au/books?id=ER0nAAAAMAAJ},
	  year={1954},
	  publisher={Interscience Publishers}
	}
	
	@article{M2002,
	author = {M. C. Liu, T. Z. Wang},
	journal = {Acta Arithmetica},
	keywords = {Vinogradov's three prime theorem; ternary {{Goldbach}}'s problem; trigonometric sums over primes; circle method},
	language = {eng},
	number = {2},
	pages = {133-175},
	title = {On the {Vinogradov} bound in the three primes {{Goldbach}} conjecture},
	url = {http://eudml.org/doc/278627},
	volume = {105},
	year = {2002},
	}
	
	@article{vinogradov1937,
	title={Representation of an odd number as a sum of three primes},
	author={I. M. Vinogradov},
	year={1937},
	journal={Dokl. Akad. Nauk. SSR 15}, 
	pages={291–294}
	}
	
	@article{helfgott2013numerical,
	  title={Numerical verification of the Ternary {{Goldbach}} Conjecture up to 8.875{\textperiodcentered} 1030},
	  author={Helfgott, Harald A and Platt, David J},
	  journal={Experimental Mathematics},
	  volume={22},
	  number={4},
	  pages={406--409},
	  year={2013},
	  publisher={Taylor \& Francis}
	}
	
	@article{deshouillers1997complete,
	  title={A complete {Vinogradov} 3-primes theorem under the {Riemann} hypothesis},
	  author={Deshouillers, J-M and Effinger, Gove and Te Riele, Herman and Zinoviev, Dmitrii},
	  journal={Electronic Research Announcements of the American Mathematical Society},
	  volume={3},
	  number={15},
	  pages={99--104},
	  year={1997}
	}
	
	@article{chen1978goldbach,
	  title={On the {Goldbach's} problem and the sieve methods},
	  author={CHEN, Jing-Run},
	  journal={Scientia Sinica},
	  volume={21},
	  number={6},
	  pages={701--739},
	  year={1978},
	  publisher={Science China Press}
	}
	
	@article{pintz2006romanov,
	  title={A note on Romanov's constant},
	  author={Pintz, J{\'a}nos},
	  journal={Acta Mathematica Hungarica},
	  volume={112},
	  number={1-2},
	  pages={1--14},
	  year={2006},
	  publisher={Springer}
	}
	
	@article{romanoff1934einige,
	  title={{\"U}ber einige S{\"a}tze der additiven Zahlentheorie},
	  author={Romanoff, NP},
	  journal={Mathematische Annalen},
	  volume={109},
	  number={1},
	  pages={668--678},
	  year={1934},
	  publisher={Springer}
	}
	
	%this citation may not be legit
	@article {selberg1952,
	    author  = {A. Selberg},
	    title   = {On elementary methods in primenumber-theory and their limitations},
	    journal = {Den 11te Skandinaviske Matematikerkongress (Trondheim, 1949), Johan Grundt Tanums Forlag, Oslo},
	    year  = {1952},
	    pages  = {13-22}
	}
	
	@article {corput1950,
  	author  = {Johannes Gaultherus van der Corput},
  	title   = {On de Polignac's Conjecture},
  	journal = {Simon Stevin},
  	year  = {1950},
  	volume= {27},
  	pages  = {99-105}
	}
	
	@article{erdos1950,
	author = {Paul Erd\"{o}s},
	title = {On integers of the form $2^k + p$ and some related problems},
	journal = {Summa Brasil. Math.},
	volume={2},
	year={1950},
	pages={113--125}
	}
	
	@article{romani1983computations,
	  title={Computations concerning primes and powers of two},
	  author={Romani, F},
	  journal={Calcolo},
	  volume={20},
	  number={3},
	  pages={319--336},
	  year={1983},
	  publisher={Springer}
	}

	@article{heath2002integers,
	  title={Integers represented as a sum of primes and powers of two},
	  author={Heath-Brown, D Roger and Puchta, J-C},
	  journal={arXiv preprint math/0201299},
	  year={2002}
	}
	
	@article{platt2015linnik,
	  title={Linnik's approximation to {{Goldbach}}'s conjecture, and other problems},
	  author={Platt, DJ and Trudgian, TS},
	  journal={Journal of Number Theory},
	  volume={153},
	  pages={54--62},
	  year={2015},
	  publisher={Elsevier}
	}
	
	@article{pintz2003linnik,
	  title={On Linnik's approximation to {Goldbach}'s problem, I},
	  author={Pintz, J and Ruzsa, IZ},
	  journal={Acta Arithmetica},
	  volume={109},
	  number={2},
	  pages={169--194},
	  year={2003}
	}
	
	@article{pintz2004goldbach,
		  title={On the representation of {Goldbach} numbers by a bounded number of powers of two},
		  author={J. Pintz and A. Khalfalah},
		  journal={Proceedings Elementary and Analytic Number Theory},
		  year={2004}
	}
	
	@article{wrench1961evaluation,
	  title={Evaluation of Artin's constant and the twin-prime constant},
	  author={Wrench Jr, John W},
	  journal={Mathematics of Computation},
	  pages={396--398},
	  year={1961},
	  publisher={JSTOR}
	}
	
	@article{chen2004romanoff,
	  title={On Romanoff's constant},
	  author={Chen, Yong-Gao and Sun, Xue-Gong},
	  journal={Journal of Number Theory},
	  volume={106},
	  number={2},
	  pages={275--284},
	  year={2004},
	  publisher={Elsevier}
	}
	
	@book{halberstam1974sieve,
	  title={Sieve methods},
	  author={Halberstam, H. and Richert, H.E.},
	  isbn={9780123182500},
	  lccn={lc74005661},
	  series={L.M.S. monographs},
	  url={https://books.google.com.au/books?id=pwXvAAAAMAAJ},
	  year={1974},
	  publisher={Academic Press}
	}
	
	@article{heath2002lectures,
	  title={Lectures on sieves},
	  author={Heath-Brown, DR},
	  journal={arXiv preprint math/0209360},
	  year={2002}
	}
	
		@book{apostol1998introduction,
		  title={Introduction to Analytic Number Theory},
		  author={Apostol, T.M.},
		  isbn={9780387901633},
		  lccn={98164861},
		  series={Undergraduate Texts in Mathematics},
		  url={https://books.google.com.au/books?id=Il64dZELHEIC},
		  year={1998},
		  publisher={Springer, New York}
		}
		
		@article{chen1973,
		author = {CHEN JING-RUN},
		title = {ON THE REPRESENTATION OF A LARGER EVEN INTEGER AS THE SUM OF A PRIME AND THE PRODUCT OF AT MOST TWO PRIMES},
		publisher = {SCIENCE CHINA Mathematics},
		year = {1973},
		journal = {SCIENCE CHINA Mathematics},
		volume = {16},
		number = {2},
		eid = {157},
		numpages = {19},
		pages = {157},
		keywords = {},
		url = {http://math.scichina.com:8081/sciAe/EN/abstract/article_380542.shtml},
		doi = {10.1360/ya1973-16-2-157}
		}    
		
		@article{Buc37,
		 author = {A.A Buchstab},
		 title= {Asymptotic estimate of one general number-theoretic function ({Russian})},
		 journal={ Mat.  Sat.},
		 year={ 1937},
		 volume= { 2 (44)},
		 issue ={ 6},
		 pages = { 1239--1246},
		 url= {http://mi.mathnet.ru/msb5649}
		}
		
		@article{hua1951estimation,
		  title={Estimation of an integral},
		  author={Hua, Loo-Keng},
		  journal={Sci. Sinica},
		  volume={4},
		  pages={393--402},
		  year={1951}
		}
		
		@article{cheer1990differential,
		  title={A differential delay equation arising from the sieve of {Eratosthenes}},
		  author={Cheer, Angela Y and Goldston, Daniel A},
		  journal={Mathematics of computation},
		  volume={55},
		  number={191},
		  pages={129--141},
		  year={1990}
		}
		
		@article{hogg1998controlling,
		  title={Controlling smart matter},
		  author={Hogg, Tad and Huberman, Bernardo A},
		  journal={Smart Materials and Structures},
		  volume={7},
		  number={1},
		  pages={R1},
		  year={1998},
		  publisher={IOP Publishing}
		}
		
		@book{book:1199806,
		   title =     {Handbook of Differential Equations},
		   author =    {Daniel Zwillinger (Auth.)},
		   publisher = {Elsevier Inc, Academic Press},
		   isbn =      {978-0-12-784391-9,0127843914},
		   year =      {1992},
		   series =    {},
		   edition =   {2nd},
		   volume =    {},
		   url =       {http://gen.lib.rus.ec/book/index.php?md5=77b5c6f3805c71373f39382bfe450a8b}
		}



@article{marsaglia1989numerical,
  title={Numerical solution of some classical differential-difference equations},
  author={Marsaglia, George and Zaman, Arif and Marsaglia, John CW},
  journal={Mathematics of Computation},
  volume={53},
  number={187},
  pages={191--201},
  year={1989}
}

@article{bruijn1950number,
  title={On the number of uncancelled elements in the sieve of Eratosthenes},
  author={de Bruijn, Nicolaas Govert},
  journal={Indag. math.},
  volume={12},
  pages={247--256},
  year={1950}
}

@book{de2012analytic,
  title={Analytic Number Theory: Exploring the Anatomy of Integers},
  author={De Koninck, J.M. and Luca, F.},
  isbn={9780821875773},
  lccn={2011051431},
  series={Graduate studies in mathematics},
  url={https://books.google.com.au/books?id=NaACAQAAQBAJ},
  year={2012},
  publisher={American Mathematical Society}
}


@article{golomb1985invincible,
  title={The Invincible Primes},
  author={Golomb, Solomon W},
  journal={The Sciences},
  volume={25},
  number={2},
  pages={50--57},
  year={1985},
  publisher={Wiley Online Library}
}

@article{liu2011density,
  title={Density of two squares of primes and powers of 2},
  author={Liu, Zhixin and L{\"U}, GUANGSHI},
  journal={International Journal of Number Theory},
  volume={7},
  number={05},
  pages={1317--1329},
  year={2011},
  publisher={World Scientific}
}

@article{habsieger2006integers,
  title={On integers of the form $p+ 2^k$},
  author={Habsieger, Laurent and Roblot, Xavier-Fran{\c{c}}ois},
  journal={Acta Arithmetica},
  volume={122},
  number={1},
  pages={45--50},
  year={2006},
  publisher={Institute of Mathematics Polish Academy of Sciences}
}

@book{stein2009real,
  title={Real analysis: measure theory, integration, and Hilbert spaces},
  author={Stein, Elias M and Shakarchi, Rami},
  year={2009},
  publisher={Princeton University Press}
}



@book{goldberg1964methods,
  title={Methods of real analysis},
  author={Goldberg, R.R.},
  lccn={lc64015980},
  series={Blaisdell book in the pure and applied sciences},
  url={https://books.google.com.au/books?id=qK8-AAAAIAAJ},
  year={1964},
  publisher={Blaisdell Pub. Co.}
}

@article{pan1964new,
  title={A new application of the Yu. V. Linnik large sieve method},
  author={Pan, Cheng-Dong},
  journal={Chinese Math. Acta},
  volume={5},
  pages={642--652},
  year={1964}
}

@article{bombieri1966small,
  title={Small differences between prime numbers},
  author={Bombieri, E and Davenport, H},
  journal={Proceedings of the Royal Society of London A: Mathematical, Physical and Engineering Sciences},
  volume={293},
  pages={1--18},
  year={1966},
  organization={The Royal Society}
}

@article{liu2000representation,
  title={Representation of even integers as sums of squares of primes and powers of 2},
  author={Liu, Jianya and Liu, Ming-Chit},
  journal={Journal of Number Theory},
  volume={83},
  number={2},
  pages={202--225},
  year={2000},
  publisher={Elsevier}
}

@article{liu1998number,
  title={The number of powers of 2 in a representation of large even integers II},
  author={Liu, Jianya and Liu, Mingchit and Wang, Tianze},
  journal={Science in China Series A: Mathematics},
  volume={41},
  number={12},
  pages={1255--1271},
  year={1998},
  publisher={Springer}
}

@article{li2000number,
  title={The number of powers of 2 in a representation of large even integers by sums of such powers and of two primes},
  author={Li, Hong Ze},
  journal={ACTA ARITHMETICA-WARSZAWA-},
  volume={92},
  number={3},
  pages={229--237},
  year={2000},
  publisher={THE INSTITUTE OF MATHEMATICS}
}

@article{li2001number,
  title={The number of powers of 2 in a representation of large even integers by sums of such powers and of two primes (II)},
  author={Li, Hongze},
  journal={Acta Arithmetica},
  volume={96},
  pages={369--379},
  year={2001},
  publisher={Instytut Matematyczny Polskiej Akademii Nauk}
}

@article{wang1999linnik,
  title={On Linnik’s almost {Goldbach} theorem},
  author={Wang, Tianze},
  journal={Science in China Series A: Mathematics},
  volume={42},
  number={11},
  pages={1155--1172},
  year={1999},
  publisher={Springer}
}

@article{liu1999almost,
  title={On the almost {Goldbach} problem of Linnik},
  author={Liu, Jianya and Liu, Ming-Chit and Wang, Tianze},
  journal={Journal de th{\'e}orie des nombres de Bordeaux},
  volume={11},
  number={1},
  pages={133--147},
  year={1999}
}

@article{linnik1953addition,
  title={Addition of prime numbers with powers of one and the same number},
  author={Linnik, Yurii Vladimirovich},
  journal={Matematicheskii Sbornik},
  volume={74},
  number={1},
  pages={3--60},
  year={1953},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian Academy of Sciences}
}

@article{linnik1951prime,
  title={Prime numbers and powers of two},
  author={Linnik, Yurii Vladimirovich},
  journal={Trudy Matematicheskogo Instituta imeni VA Steklova},
  volume={38},
  pages={152--169},
  year={1951},
  publisher={Russian Academy of Sciences, Steklov Mathematical Institute of Russian Academy of Sciences}
}

@article{o2009genuine,
  title={The genuine sieve of Eratosthenes},
  author={O'NEILL, MELISSA E},
  journal={Journal of Functional Programming},
  volume={19},
  number={01},
  pages={95--106},
  year={2009},
  publisher={Cambridge Univ Press}
}

@article{dongwrong,
	title={An improvement of J. R. Chen's theorem},
    author={Wu, Dong Hua},
    journal={Shanghai Keji Daxue Xuebao},
    year={1997},
    pages={94--99},
    }
    
@article{tim_email,
	title={Personal Correspondance},
	author={Trudgian, Tim and Wu, Jie},
	year={2013},
	}
	
		@article{yamada2015explicit,
		  title={Explicit Chen's theorem},
		  author={Yamada, Tomohiro},
		  journal={arXiv preprint arXiv:1511.03409},
		  year={2015}
		}
	
	@article{friedlander1991oscillation,
	  title={Oscillation theorems for primes in arithmetic progressions and for sifting functions},
	  author={Friedlander, John and Granville, Andrew and Hildebrand, Adolf and Maier, Helmut},
	  journal={Journal of the American Mathematical Society},
	  volume={4},
	  number={1},
	  pages={25--86},
	  year={1991},
	  publisher={JSTOR}
	}
	
	@article{iwaniec1980new,
	  title={A new form of the error term in the linear sieve},
	  author={Iwaniec, Henryk},
	  journal={Acta Arithmetica},
	  volume={37},
	  number={1},
	  pages={307--320},
	  year={1980}
	}
	
	@article{fliegel1989goldbach,
	  title={{Goldbach}'s Comet: the numbers related to {Goldbach}'s Conjecture},
	  author={Fliegel, Henry F and Robertson, Douglas S},
	  journal={Journal of Recreational Mathematics},
	  volume={21},
	  number={1},
	  pages={1--7},
	  year={1989}
	}
	
	@article{baker2007excel,
	  title={Excel and the {Goldbach} comet},
	  author={Baker, John},
	  journal={Spreadsheets in Education (eJSiE)},
	  volume={2},
	  number={2},
	  pages={2},
	  year={2007}
	}
	
	@book{stewart2015calculus,
	  title={Calculus},
	  author={Stewart, James},
	  year={2015},
	  publisher={Cengage Learning}
	}
	
	@article{burden1985numerical,
	  title={Numerical analysis (1985)},
	  author={Burden, RL and Faires, Je D and Reynolds, AC},
	  journal={Prindle, Weber \& Schmidt},
	  year={1985}
	}
	


==> dedication.tex <==


\blanknonumber\ \blanknonumber

\vspace*{\fill}

\begin{center}\emph{
%
For Sarah
%
}
\end{center}

\vfill\vfill\vfill

